A Variational View on Bootstrap Ensembles as Bayesian Inference

In this paper, we employ variational arguments to establish a connection between ensemble methods for Neural Networks and Bayesian inference. We consider an ensemble-based scheme where each model/particle corresponds to a perturbation of the data by means of parametric bootstrap and a perturbation of the prior. We derive conditions under which any optimization steps of the particles makes the associated distribution reduce its divergence to the posterior over model parameters. Such conditions do not require any particular form for the approximation and they are purely geometrical, giving insights on the behavior of the ensemble on a number of interesting models such as Neural Networks with ReLU activations. Experiments confirm that ensemble methods can be a valid alternative to approximate Bayesian inference; the theoretical developments in the paper seek to explain this behavior.

==> classification.tex <==

\subsection{Extensions to Classification}

Regarding the problem of classification, it is not obvious how to identify a data resampling strategy in the style of our approach to regression. 
We seek to create data replicates from a parametric distribution that reflects the properties of the Bernoulli likelihood.
Assume that a class label $y$ can take values in $\{0, 1\}$; if we locally fit a distribution $\mathrm{Bern}(p)$ to each $y$, the \ML parameter will be the one-sample mean i.e.\ $p_* = 0$ or $p_* = 1$.
The act of resampling from such a fitted model will deterministically produce either $0$ or $1$, eliminating thus any chance of perturbing the data.

Nevertheless, we think that classification can still benefit from bootstrapping.
Although an in-depth exploration of ensemble-based classification is out of the scope of this work,
we demonstrate how a Gaussian-based perturbation can be extended to classification by employing local Gaussian approximations to the likelihood in the style of \cite{MiliosNIPS}.
In this way, we effectively turn classification into a regression problem in a latent space (see Section \ref{sec:classif_suppl} of the supplement).

%More specifically, each Bernoulli likelihood will be regarded as a degenerate beta distribution, to which we add a small regularisation term $\alpha_\epsilon = 0.01$.
%In this way, the labels ``$0$'' will be represented as $\mathrm{Beta}(\alpha_\epsilon, 1+\alpha_\epsilon)$, while the labels ``$1$'' as $\mathrm{Beta}(1+\alpha_\epsilon, \alpha_\epsilon)$.
%Classification is then treated as two parallel regression problems on the observed parameters of the beta distributions, for which we assume Gamma likelihoods\footnote{We leverage the fact that a beta-distributed random variable $x\sim \mathrm{Beta}(a,b)$ can be constructed as the ratio Gamma-distributed variables i.e.\ $x = x_a/(x_a+x_b)$, where $x_a \sim \mathrm{Gamma}(a, 1)$ and $x_b \sim \mathrm{Gamma}(b, 1)$.}.
%The next step is to locally approximate the Gamma likelihood models with log-Normals by means of moment matching, which eventually translates to a regression problem with Gaussian likelihood in the log space.
%Learning can be performed in this latent space and any predictions can be mapped back into probabilities by the soft-max function.

\begin{figure}
	\centering
	\includegraphics[width=\linewidth]{figs/demo_classif_relu.pdf}
	\caption{Application of Bootstrap to Classification. 
		%Left: only the prior is perturbed. Middle: the classification labels are perturbed along with the prior. Right: samples from \mcmc
	}
	\label{fig:demo_classif}
\end{figure}


Figure \ref{fig:demo_classif} illustrates an example of applying parametric bootstrap to a synthetic classification problem, considering one hidden layer and \relu activations.
The shaded areas represent the 95\% support of the sampled distributions of classifiers.
The combination of bootstrap with locally approximated likelihoods on the left produces a fairly accurate approximation of the \mcmc result on the right.


%When the likelihood approximation trick is applied, the resulting distribution better approximated the result of MCMC.
%We see that if labels are not perturbed, the predictive variance becomes very small near the regime of observed values, even if we apparently have an informative quantification of uncertainty in areas where no data-point are observed.



